Probabilistic learning of nonlinear dynamical systems using sequential Monte Carlo

Probabilistic modeling provides the capability to represent and manipulate uncertainty in data, models, predictions and decisions. We are concerned with the problem of learning probabilistic models of dynamical systems from measured data. Specifically, we consider learning of probabilistic nonlinear state-space models. There is no closed-form solution available for this problem, implying that we are forced to use approximations. In this tutorial we will provide a self-contained introduction to one of the state-of-the-art methods---the particle Metropolis--Hastings algorithm---which has proven to offer a practical approximation. This is a Monte Carlo based method, where the particle filter is used to guide a Markov chain Monte Carlo method through the parameter space. One of the key merits of the particle Metropolis--Hastings algorithm is that it is guaranteed to converge to the "true solution" under mild assumptions, despite being based on a particle filter with only a finite number of particles. We will also provide a motivating numerical example illustrating the method using a modeling language tailored for sequential Monte Carlo methods. The intention of modeling languages of this kind is to open up the power of sophisticated Monte Carlo methods---including particle Metropolis--Hastings---to a large group of users without requiring them to know all the underlying mathematical details.

==> planIntro.tex <==



Provide the feeling that they do not have to implement all of this on their own. We are making solutions available via a 
new programming language that is designed to solve these problems. Throughout the paper we will illustrate this with 
examples using a prototype of this language.

The aim of the tutorial is to proved sufficient knowledge about the underlying methods 
such that you as a reader should feel comfortable in using the language for solving problems of these kind. The language 
will serve the important purpose of abstracting away the underlying mathematics from the user allowing them to focus 
on their problem at hand instead.
\ts{How hard should we ``sell'' the tool? (i.e. Birch)}


============================================


% Background and motivation
%

1. The problem we are interested in is how to solve the nonlinear system identification problem. 
        * The first step in the extraction of knowledge from data often amounts to finding the unknown parameters in the 
           model using the data that we have available.
        * To do this the learning system needs links between the latent and the observed data. The links are made via assumptions 
           and taken together these assumptions constitute the model.
        * A mathematical model is a compact representation (set of assumptions) of the data that in precise mathematical form
           captures the key properties of the underlying system. (more specifically a model = probability distribution)
        * Probabilistic modelling
                    * Probabilistic modeling allow for representing and manipulating uncertainty in data, models, decisions and predictions. 
                       The capability of mathematically representing and manipulating uncertainty which is essential to our development is 
                       provided by probability theory. % Probability theory explains how to mathematically represent and manipulate uncertainty. \cite{Ghahramani:2015}       
                    * Uncertainty plays a fundamental role since any reasonable model will be uncertain when making predictions of unobserved data.
                    * model = probability distribution.



Give a pitch for the probabilistic (Bayesian) approach to modelling.
     * Two questions: (Why bother about stochastic nonlinear systems)
     * Why is it important to be able to account for uncertainty?
     * Why do we need to deal with nonlinear systems.
           * Pragmatic answer: ``because it gives better results and we can do it''



2. There are no closed form expressions available for this problem, which means that we are forced to approximations of some sort. The nature of the approximations we will make use of in this tutorial have the appealing property that they will converge towards the true solution the more computations we make use of. (Using sequential Monte Carlo (SMC) allows us to solve ``the right problem''.)


Introduce the model gently and thoroughly explain what the two equations stand for:
     * Talk about the dynamics as a simulator that simulates the systems one step forward. Moreover, it is a stochastic simulator.
     * The measurement model often describes a sensor of some kind.


% Contribution of this paper
%
A ``specific tutorial'' in the sense that we provide an introduction to one powerful ``combination of SMC+MCMC'' (possibly too detailed).
rather than surveying all available methods, see e.g. \cite{Schon, Kantas:} for such accounts.
In the accompanying paper~\cite{SvenssonLS:2017abc} we show how probabilistic modelling implemented via the techniques outlined in this tutorial are used to solve ``one of the challenging benchmark problems'' with promising results.

One advantage of the particular algorithm ``we put forward'' is that it only requires us to be able to simulate the model. (Explain why 
this is interesting and what it means, give a few examples).


% Outline
% 


